Disentangling the AGN and Star-Formation Contributions to the Radio-X-ray Emission of Radio-Loud Quasars at 1<z<2

We constrain the emission mechanisms responsible for the prodigious electromagnetic output generated by active galactic nuclei (AGN) and their host galaxies with a novel state-of-the-art AGN radio- to-X-ray spectral energy distribution model fitting code (ARXSED). ARXSED combines multiple components to fit the spectral energy distributions (SEDs) of AGN and their host galaxies. Emission components include radio structures such as lobes and jets, infrared emission from the AGN torus, visible-to-X-ray emission from the accretion disk, and radio-to-ultraviolet emission from the host galaxy. Applying ARXSED to the radio SEDs of 20 3CRR quasars at 1 < z < 2 verifies the need for more than a simple power law when compact radio structures are present. The non-thermal emission contributes 91%-57% of the observed-frame 1.25mm to 850{\mu}m flux, and this component must be accounted for when using these wavelengths to estimate star-formation properties. We predict the presence of strong radio-linked X-ray emission in more than half the sample sources. ARXSED estimates median (and the associated first and third quartile ranges) BH mass of $2.9_{1.7}^{6.0} \times 10^9~\rm M_{\odot}$, logarithm of Eddington ratio of $ -1.0_{-1.2}^{-0.6} $, and spin of $ 0.98_{0.94}^{0.99} $ for our sample. The inferred AGN torus and accretion disk parameters agree with those estimated from spectroscopic analyses of similar samples in the literature. We present the median intrinsic SED of the luminous radio-loud quasars at 1 < z < 2 ; this SED represents a significant improvement in the way each component is modeled.

==> table.tex <==
\begin{table*}[]
\begin{turn}{0}
\begin{tabular}
{|c| c| c| c| c| c| c| c| c| c| c| c| c| c| c| c| c|}
    \hline 
ID& $f_{7.22} $& $f_{7.26} $& $f_{7.27} $& $f_{7.34} $& $f_{7.38} $& $f_{7.41} $& $f_{7.42} $& $f_{7.45} $& $f_{7.50} $& $f_{7.58} $& $f_{7.78} $& $f_{7.87} $& $f_{7.90} $& $f_{7.93} $& $f_{8.18} $& $f_{8.25}$\\\hline

3C9 &  & 129. &  &  &  &  &  &  &  & 75.5 & 53.0 &  &  & 35.7 &  & 16.3\\\hline
3C14 &  &  &  &  &  &  &  &  & 55.7 &  &  &  &  & 24.4 &  & 11.3\\\hline
3C43 &  &  &  &  &  &  &  & 54.1 &  &  &  &  & 23.0 &  &  & 12.7\\\hline
3C181 &  &  &  &  &  &  &  &  & 47.7 &  & 54.0 &  &  & 24.2 &  & 15.8\\\hline
3C186 &  &  &  &  &  & 62.0 &  &  &  &  & 42.0 &  &  & 33.2 & 15.6 & 15.4\\\hline
3C190 &  &  &  & 79.2 &  &  &  &  &  &  &  &  &  & 26.8 &  & 16.4\\\hline
3C191 & 165. &  &  &  &  &  &  &  &  & 56.6 &  &  &  & 34.3 &  & 14.2\\\hline
3C204 &  &  & 145. &  &  &  &  &  &  &  &  &  &  & 34.3 &  & 14.2\\\hline
3C205 &  & 98.7 &  &  &  &  &  &  &  &  &  &  &  & 39.2 &  & 13.7\\\hline
3C208 &  &  &  &  &  &  &  & 74.8 &  &  & 42.0 &  &  & 41.5 &  & 20.2\\\hline
3C212 &  &  &  &  &  &  &  &  &  &  & 46.0 &  &  & 29.8 &  & 16.5\\\hline
3C245 &  & 103. &  &  &  &  &  &  &  &  & 34.0 &  &  & 27.4 &  & 15.7\\\hline
3C268.4 &  &  &  &  &  &  &  &  & 36.2 &  &  & 20.7 &  & 22.4 &  & 11.2\\\hline
3C270.1 &  &  &  &  & 73.0 &  &  &  &  &  &  &  &  & 30.8 &  & 14.8\\\hline
3C287 &  &  &  &  &  &  &  &  &  & 31.5 &  &  &  & 19.4 & 15.5 & 17.5\\\hline
3C318 &  &  &  &  &  &  &  & 32.1 &  &  &  &  &  & 23.5 & 14.0 & 13.4\\\hline
3C325 &  &  &  &  &  &  &  &  &  & 43.7 &  &  &  & 33.1 &  & 17.0\\\hline
4C16.49 &  &  &  &  &  &  & 43.2 &  &  &  &  &  &  &  &  & 10.5\\\hline
3C432 &  &  &  &  & 53.9 &  &  &  &  & 55.4 &  &  &  & 21.1 &  & 12.0\\\hline
3C454.0 &  &  &  &  &  &  &  &  &  & 31.8 & 24.0 &  &  &  &  & 12.7\\\hline
   
    \end{tabular}
    \end{turn}
    \end{table*}



\begin{table*}[]
\begin{turn}{0}
\begin{tabular}
{|c| c| c| c| c| c| c| c| c| c| c| c| c| c|} \hline
 ID & $f_{8.56} & $f_{8.61} & $f_{8.88} & $f_{9.15} & $f_{9.43} & $f_{9.69} & $f_{9.70} & $f_{9.91} & $f_{9.95} & $f_{10.0} & $f_{10.2} & $f_{10.5} & $f_{11.0}$\\\hline
 3C9 &  & 7.78 & 3.89 & 1.96 & 0.980 &  & 0.546 &  &  & 0.216 & 0.130 &  & \\\hline
3C14 & 6.83 &  & 3.58 & 1.87 & 1.02 &  & 0.606 &  &  & 0.216 & 0.150 &  & \\\hline
3C43 &  & 6.43 & 4.28 & 2.82 & 1.70 &  & 1.08 &  &  & 0.611 & 0.450 &  & 0.189\\\hline
3C181 & 7.63 &  & 3.76 & 2.31 & 1.25 &  & 0.655 &  &  & 0.291 & 0.200 &  & \\\hline
3C186 & 6.59 &  & 2.74 & 1.24 & 0.585 & 0.308 &  &  &  & 0.0841 &  &  & \\\hline
3C190 & 9.09 &  & 4.30 & 2.55 & 1.39 &  & 0.814 &  &  & 0.356 & 0.300 &  & \\\hline
3C191 & 7.49 &  & 3.44 & 1.85 & 0.959 &  & 0.457 &  &  & 0.225 & 0.180 &  & \\\hline
3C204 & 7.49 &  & 3.44 & 1.84 & 0.505 &  & 0.338 &  &  & 0.159 & 0.110 &  & \\\hline
3C205 & 9.28 &  & 3.95 & 2.39 & 1.12 &  & 0.665 &  &  & 0.234 & 0.160 &  & \\\hline
3C208 & 10.3 &  & 4.56 & 2.37 & 0.959 &  & 0.536 &  &  & 0.234 & 0.140 &  & \\\hline
3C212 & 8.34 &  & 4.44 & 2.37 & 1.42 &  & 0.884 &  &  & 0.497 & 0.480 &  & 0.106\\\hline
3C245 & 9.46 &  & 5.06 & 3.31 & 2.19 &  & 1.38 &  & 1.04 & 0.967 & 0.850 & 0.940 & \\\hline
3C268.4 & 6.59 &  & 3.62 & 1.98 & 1.07 &  & 0.596 &  &  & 0.244 & 0.180 &  & \\\hline
3C270.1 & 9.75 &  & 5.04 & 2.73 & 1.50 &  & 0.864 &  &  & 0.450 & 0.440 &  & \\\hline
3C287 & 15.0 &  & 9.67 & 7.06 & 4.65 &  & 3.24 & 2.20 &  & 1.73 & 1.42 &  & 0.512\\\hline
3C318 & 9.22 &  & 4.44 & 2.56 & 1.34 &  & 0.745 &  &  & 0.319 & 0.230 &  & \\\hline
3C325 & 12.1 &  & 6.19 & 3.57 & 1.86 & 1.05 &  &  &  & 0.394 & 0.250 &  & \\\hline
4C16.49 & 6.27 & 5.36 &  & 1.46 &  & 0.345 &  &  &  &  &  &  & \\\hline
3C432 & 6.49 &  & 2.90 & 1.58 & 0.767 & 0.407 &  &  &  & 0.131 & 0.0800 &  & \\\hline
3C454.0 & 6.49 &  & 3.46 & 2.14 & 1.22 &  & 0.784 &  &  & 0.394 & 0.300 &  & \\\hline

    \end{tabular}
    \end{turn}
       \vspace{30em}
    \end{table*}
    

